Turn-taking and Backchannel Prediction with Acoustic and Large Language Model Fusion

We propose an approach for continuous prediction of turn-taking and backchanneling locations in spoken dialogue by fusing a neural acoustic model with a large language model (LLM). Experiments on the Switchboard human-human conversation dataset demonstrate that our approach consistently outperforms the baseline models with single modality. We also develop a novel multi-task instruction fine-tuning strategy to further benefit from LLM-encoded knowledge for understanding the tasks and conversational contexts, leading to additional improvements. Our approach demonstrates the potential of combined LLMs and acoustic models for a more natural and conversational interaction between humans and speech-enabled AI agents.

==> Table/History.tex <==
\begin{table}[t!]
\centering
\caption{Results for instruction fine-tuning with dialogue history.}
\vskip -1em
\resizebox{\linewidth}{!}{
\label{tab:history}
\begin{tabular}{cccccc}
\hline
 Method    &   {AUC(Cont)} & AUC(Back) & AUC(Turn)  & AUC(avg)       & EER(avg)      \\
 \hline
RedPajama + History               & 0.8747 & 0.8074 &   0.8912     & 0.8578      & 21.63    \\
+ Hubert Opt1 &  \textbf{0.9029}  & \textbf{0.8184} &  \textbf{0.9197}  & \textbf{0.8803}     &\textbf{19.3}    \\
\hline
\end{tabular}
}
\end{table}
